Tight Logarithmic Separations between LZ77 and LZRR

LZRR is a copy-based lossless compression method that produces a bidirectional macro scheme. It greedily parses a string from left to right. At each step, it can copy from an occurrence on either side of the current position, provided that the copy creates no cycle. Let $z$ and $z_{\mathrm{RR}}$ denote the sizes of the LZ77 and LZRR parsings, respectively. Under the original LZRR rule, we show that $z/z_{\mathrm{RR}}=\Theta(\log n)$ on a family of Fibonacci words and that $z_{\mathrm{RR}}/z=\Theta(\log n)$ on a family based on bit reversal, where $n$ is the string length. The Fibonacci separation holds under every tie-breaking rule. Both separations are asymptotically tight.

==> theorems.tex <==
\RequirePackage{amsthm}
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{property}[theorem]{Property}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}

